RAM: Reachability Across Morphologies

Many stages of the robotic lifecycle, from morphology synthesis to operation, rely fundamentally on the reachable workspace. However, current methods for approximating workspaces are slow, imprecise, or tied to a single morphology. We introduce Reachability Across Morphologies (RAM): a morphology-conditioned, implicit neural representation that acts as a fast, differentiable surrogate for pose reachability, generalising to unseen morphologies while inherently accounting for self-collisions. RAM is trained on a large-scale dataset of $3\cdot10^{10}$ samples generated solely from forward kinematics, which we publish alongside the model. Experiments show that RAM reaches 84\% balanced accuracy at nanosecond inference, 15 percentage points higher than a generative inverse kinematics baseline that also generalises across morphologies, while running three orders of magnitude faster. This speed carries over to downstream tasks, accelerating morphology and trajectory optimisation by one to two orders of magnitude.

==> floats/source/hero/metrics_bars.tex <==
\begin{tikzpicture}[x=\herounit, y=\herounit]
  \pgfmathsetmacro{\W}{1.93}
  \pgfmathsetmacro{\H}{0.25}
  \pgfmathsetmacro{\gap}{0.30}
  % ── BAR 1: Reachable poses (93.54 % TP | 6.46 % FP) ───────────────────────
  \pgfmathsetmacro{\spI}{0.9354*\W}
  \fill[SNSGreen] (0,0)    rectangle (\spI, \H);
  \fill[SNSRed]   (\spI,0) rectangle (\W,   \H);
  \node[card label, text=white] at ({\W/2}, {\H/2}) {Reachable poses};
  \draw[cardborder, line width=0.4pt] (\spI, {-0.08}) -- (\spI, {0.0});
  \node[card label, text=SNSGreen, anchor=east] at ({\spI-0.01}, {-0.1}) {TP};
  \node[card label, text=SNSRed,   anchor=west] at ({\spI+0.01}, {-0.1}) {FN};
  % ── BAR 2: Unreachable poses (73.75 % TN | 26.25 % FN) ────────────────────
  \pgfmathsetmacro{\xo}{\W+\gap}
  \pgfmathsetmacro{\spII}{0.7375*\W}
  \fill[SNSGreen] ({\xo},       0) rectangle ({\xo+\spII}, \H);
  \fill[SNSRed]   ({\xo+\spII}, 0) rectangle ({\xo+\W},    \H);
  \node[card label, text=white] at ({\xo+\W/2}, {\H/2}) {Unreachable poses};
  \draw[cardborder, line width=0.4pt] ({\xo+\spII}, {-0.08}) -- ({\xo+\spII}, {0.0});
  \node[card label, text=SNSGreen, anchor=east] at ({\xo+\spII-0.01}, {-0.1}) {TN};
  \node[card label, text=SNSRed,   anchor=west] at ({\xo+\spII+0.01}, {-0.1}) {FP};
\end{tikzpicture}
